Addressing Over-Smoothing in Graph Neural Networks via Deep Supervision

Learning useful node and graph representations with graph neural networks (GNNs) is a challenging task. It is known that deep GNNs suffer from over-smoothing where, as the number of layers increases, node representations become nearly indistinguishable and model performance on the downstream task degrades significantly. To address this problem, we propose deeply-supervised GNNs (DSGNNs), i.e., GNNs enhanced with deep supervision where representations learned at all layers are used for training. We show empirically that DSGNNs are resilient to over-smoothing and can outperform competitive benchmarks on node and graph property prediction problems.

==> content/experiments.tex <==
\section{Empirical Evaluation}
\label{sec:empirical_evaluation}

%\subsection{Experiments}
%\label{sec:experiments}
We aim to empirically evaluate the performance of DSGNNs on a number of challenging graph and node classification and regression tasks. 
%For these datasets, \cite{errica2019fair} showed  that baseline algorithms that do not use the graph structure easily outperform those that do; that is, GNNs fail to effectively use the available structure. 
We investigate empirically if the addition of deep supervision provides an advantage over the standard GNN and JKNet \citep{jumping-knowledge-networks-xu18c} architectures shown in  \cref{fig:gnn_architectures}. 

We implemented\footnote{We will release the source code upon publication acceptance} the standard GNN, JKNet, and DSGNN architectures using PyTorch and the Deep Graph Library  \citep[DGL,][]{wang2019dgl}. The version of the datasets we use is that available via DGL\footnote{\url{https://github.com/dmlc/dgl}} and DGL-LifeSci\footnote{\url{https://github.com/awslabs/dgl-lifesci}}. All experiments were run on a workstation with $8$GB of RAM, Nvidia Telsa P100 GPU, and Intel Xeon processor.
\begin{table}[ht]
    \caption{Graph regression and classification performance for the standard GNN, JKNet, and DSGNN architectures. The performance metric is mean test RMSE for \esol and \lipo and mean test accuracy for \enzymes calculated using $10$ repeats of $10$-fold cross validation. Standard deviation is given in parenthesis and the model depth that achieved the best performance in square brackets. Bold and underline indicate the best and second best models for each dataset.}
    \vskip 0.15in
    \begin{center}
    \begin{small}
    % \begin{sc}
    \begin{tabular}{llll}
        \toprule
        Model &  \esol & \lipo & \enzymes \\ 
              &   \multicolumn{2}{c}{RMSE $\downarrow$} & \multicolumn{1}{c}{Accuracy $\uparrow$} \\
        \midrule
        GNN     &  \underline{0.726}             & \underline{0.618}           & \underline{64.1} \\
                &  \underline{(0.063) [6]}       & \underline{(0.033) [8]}     & \underline{(6.8) [2]} \\
        JKNet   &  0.728                         & 0.633                       & \textbf{65.7}  \\ 
                &  (0.074) [8]                   & (0.035) [10]                & \textbf{(5.8) [2]}  \\ 
        DSGNN   &  \textbf{0.694}                & \textbf{0.594}              & 63.3 \\ 
                &  \textbf{(0.065) [16]}         & \textbf{(0.033) [16]}       & (7.7) [2] \\ 
        \bottomrule
    \end{tabular}
    \label{tab:results_summary_graph_datasets}
    % \end{sc}
    \end{small}
    \end{center}
    \vskip -0.15in
\end{table}
\begin{table}[ht]
    \caption{Node classification performance for  the standard GNN, JKNet, and DSGNN architectures with and without PairNorm (PN). The performance metric is mean test accuracy calculated  over $20$ repeats of fixed train/val/test splits. Standard deviation is given in parenthesis and the model depth that achieved the best performance in square brackets. Bold and underline indicate the best and second best performing models for each dataset.}
    \vskip 0.15in
    \begin{center}
    \begin{small}
    % \begin{sc}
    \begin{tabular}{l  l  l  l}
        \toprule
        Model &  \cora & \citeseer & \pubmed \\ 
              &  \multicolumn{3}{c}{Accuracy $\uparrow$} \\
        \midrule
        GNN        &   \textbf{82.6}        &  \textbf{71.1}             & \underline{77.2} \\
                   &   \textbf{(0.6) [2]}      &  \textbf{(00.6) [2]}    & \underline{(0.5) [9]} \\
        JKNet      &   \underline{81.4}        &  68.5                   & 76.9  \\ 
                   &   \underline{(0.6) [3]}   &  (0.4) [2]              & (0.9) [11] \\         
        DSGNN      &   81.1                    &  \underline{69.9}       & \textbf{77.5} \\ 
                   &   (1.0) [4]               &  \underline{(0.4) [3]}  & \textbf{(0.5) [12]} \\ 
        GNN-PN     &   77.9                    &  68.0                   & 75.5 \\
                   &   (0.4) [2]               &  (0.7) [3]              & (00.7) [15] \\        
        DSGNN-PN   &   73.1                    &  59.4                   & 75.9  \\ 
                   &   (0.8) [7]               &  (1.6) [2]              & (00.5) [7] \\         
        \bottomrule
    \end{tabular}
    \label{tab:results_summary_node_datasets}
    % \end{sc}
    \end{small}
    \end{center}
    \vskip -0.15in
\end{table}
\begin{table}[ht]
    \caption{\textbf{Missing features setting} node classification performance comparison between the standard GNN, JKNet and DSGNN architectures with and without PairNorm (PN). Results shown are mean test accuracy and standard deviation over $20$ repeats of fixed train/val/test splits. In parenthesis we indicate the model depth that achieved the highest accuracy. Bold and underline indicate the best and second best performing models.}
    \vskip 0.15in
    \begin{center}
    \begin{small}
    % \begin{sc}
    \begin{tabular}{l  l  l  l}
        \toprule
        Model &  \cora & \citeseer & \pubmed \\ 
              &  \multicolumn{3}{c}{Accuracy $\uparrow$} \\
        \midrule
        GNN        &  \textbf{77.5}             &   \textbf{62.8}                 &  \underline{76.8} \\
                   &  \textbf{(0.8) [10]}       &   \textbf{(0.7) [2]}            &  \underline{(0.7) [9]} \\        
        JKNet      &  74.9                      &   61.8                          &  76.4  \\ 
                   &  (1.0) [15]                &   (0.8) [2]                     &  (0.7) [9] \\         
        DSGNN      &  \underline{76.8}          &   61.0                          &  \textbf{0.771} \\ 
                   &  \underline{(0.8) [11]}    &   (1.0) [2]                     &  \textbf{(0.4) [10]} \\         
        GNN-PN     &  75.8                      &   \underline{62.1}              &  75.0 \\
                   &  (0.4) [6]                 &   \underline{(0.6) [4]}         &  (0.7) [15] \\        
        DSGNN-PN   &  73.5                      &   52.8                          &  74.7 \\ 
                   &  (0.9) [15]                &   (1.2) [9]                     &  (0.9) [25] \\         
        \bottomrule
    \end{tabular}
    \label{tab:results_summary_node_datasets_mv}
    % \end{sc}
    \end{small}
    \end{center}
    \vskip -0.15in
\end{table}

\subsection{Datasets and Experimental Set-up}
\label{sec:datasets}

DSGNN is a general architecture such that it can use any combination of graph convolutional and readout layers. We focus the empirical evaluation on a small number of representative methods. For graph convolutions we use graph attention networks \citep[GAT,][]{velickovic2018graph} with multi-head attention
%, as they have been shown by \citet{dwivedi2020benchmarking} to be more expressive than the standard GCN architecture of \citet{kipf2016semi}. 
We average or concatenate the outputs of the attention heads (we treat this operation as a hyper-parameter) and use the resulting node vectors as input to the next layer.

For DSGNN and JKNet, the last GAT layer is followed by a fully connected layer with an activation suitable for the downstream task, e.g., softmax for classification. The linear layer is necessary to map the GAT layer representations to the correct dimension for the downstream task. So, a DSGNN or JKNet model with $K$ layers comprises of $K-1$ GAT layers and one linear layer. For a standard GNN model, the last layer is also GAT following \citet{velickovic2018graph} such that a $K$-layer model comprises of $K$ GAT layers.

We used the evaluation protocol proposed by~\citet{errica2019fair} and present results for six benchmark datasets. Of these, three are graph tasks and three are node tasks. We include detailed dataset statistics in Table \ref{tab:datasets} in the Appendix.

\subsubsection{Graph Property Prediction}
\label{sec:graph_regression_datasets}

The graph property prediction datasets are from biochemistry where graphs represent molecules. The task is to predict molecular properties. We base our empirical evaluation on three datasets which are ESOL from \citet{delaney2004esol}, Lipophilicity from \citet{gaulton2017chembl} and \enzymes from \citet{schomburg2004brenda}. \enzymes is a graph classification task whereas \esol and \lipo are regression tasks. We use $10$-fold cross validation and repeat each experiment $10$ times. We optimize the root mean square error (RMSE) for regression and the cross-entropy loss for classification.
%Splitting is performed uniformly at random as proposed by~\citet{wu2018moleculenet}.

For all architectures, we set all hidden layers to size $512$ with $4$ attention heads (total $2048$ features). All layers are followed with a $\relu$ activation~\citep{nair2010rectified} except the last one; the last layer either uses $\softmax$ activation or no activation for classification and regression tasks respectively. We varied model depth in the range $\{ 2,4,6,\ldots,20 \}$. For readout, we use the non-parametric max function. We perform grid search for learning rate: \{$0.01$, $0.001$, $0.0001$\} and weight decay: \{$0.001$, $0.0001$\}. We use batch size $64$ and train for a maximum $500$ epochs using mini-batch SGD with momentum set to $0.9$.
% For readout, we evaluate the non-parametric mean and max functions as well as the parametric gated self-attention from~\cite{ilse2018attention}. For attention-based readout we consider two different attention sizes $64$ and $128$. We do not consider readout functions that coarsen the graph although deep supervision would still be applicable. Lastly, for the classification datasets, we tuned the learning rate over the range \{$0.01, 0.001, 0.0005, 0.0001$\} and set the number of training epochs to $300$; we also halved the learning rate every $100$ epochs and used a fixed batch size of $10$. For the regression datasets, we used learning rate $0.001$, training epochs $100$, batch size $64$ and and halved the learning rate every $20$ epochs. 
\subsubsection{Node Property Prediction}
\label{sec:node_classification_datasets}

The node classification datasets are the citation networks \cora, \citeseer and \pubmed from \citet{sen2008collective}. The task for all datasets is semi-supervised node classification in a regime with few labeled nodes. We used the splits from \citet{yang2016revisiting} and performance on the validation set for hyper-parameter selection. We repeat each experiment $20$ times. We optimize the cross-entropy loss and use accuracy for model selection and performance comparison.

We set all hidden layers to size $8$ with $8$ attention heads (total $64$ features) and $\elu$~\citep{clevert2015fast} activation for all GAT layers. We varied model depth in the range $\{ 2,3,\ldots,12,15,20,25 \}$. We performed grid search for the initial learning rate: \{$0.01, 0.002, 0.005$\}, weight decay: \{$0.0, 0.005, 0.0005$\}, and dropout (both feature and attention): \{$0.2, 0.5$\}. We trained all models using the Adam optimiser~\citep{kingma2014adam} for a maximum $1000$ epochs and decayed the learning rate by a factor of $0.5$ every $250$ epochs.
\begin{figure*}[t]
	\centering
	    \begin{tabular}{c}
        	\includegraphics[width=16.5cm]{figures/graph_results.pdf} \\
        \end{tabular}
    \caption{Graph classification and regression performance of standard GNN, JKNet, and DSGNN architectures as a function of model depth. Results shown are for the \esol (left), \lipo (middle) and \enzymes (right) datasets. The performance metric for \esol and \lipo is test RMSE and for \enzymes test accuracy. All metrics are mean over $10$ runs with $1$ standard deviation error bars.}
	\label{fig:deep_gnn_graph_performance}
	\vskip -0.1in
\end{figure*}
\begin{figure*}[t]
	\centering
	    \begin{tabular}{c}
        	\includegraphics[width=16.5cm]{figures/node_classification_results.pdf} \\
        \end{tabular}
    \caption{Node classification performance comparison of standard GNN, JKNet, and DSGNN with and without PairNorm (PN) architectures as a function model depth. Results shown are for Cora (left), Citeseer (middle), and Pubmed (right) datasets. The performance metric is mean test over $20$ runs with $1$ standard deviation error bars.}
	\label{fig:deep_gnn_node_performance}
\end{figure*}
\begin{figure*}[t]
	\centering
	    \begin{tabular}{c}
        	\includegraphics[width=16.5cm]{figures/node_classification_mv_results.pdf} \\
        \end{tabular}
    \caption{\textbf{Missing features setting} node classification performance comparison of standard GNN, JKNet, and DSGNN with and without PairNorm (PN) architectures as a function model depth. Results shown are for Cora (left), Citeseer (middle), and Pubmed (right) datasets. The performance metric is mean test over $20$ runs with $1$ standard deviation error bars.}
	\label{fig:deep_gnn_node_mv_performance}
	\vskip -0.1in
\end{figure*}

\subsection{Results}
\label{sec:results}

Tables \ref{tab:results_summary_graph_datasets} and \ref{tab:results_summary_node_datasets} show the performance for each architecture and for the all datasets. Also shown for each model is the number of layers required to achieve the best performance. For each dataset, model selection across model depth is based on validation set performance and the tables report performance on the test set for the selected models.   

\subsubsection{Graph Regression and Classification}
\label{sec:results_graph_regression_and_classification}

We see in \cref{tab:results_summary_graph_datasets} that for \esol and \lipo, models enhanced with deep supervision achieved the best outcome. In addition, DSGNN performs best at a much larger depth than the other architectures. On the graph classification dataset (\enzymes), all models perform similarly with JKNet having a small advantage. For graph classification, all architectures performed best using only $2$ convolutional layers. %; model depth provided no advantage to any of the architectures. 

Figure~\ref{fig:deep_gnn_graph_performance} shows the performance of each architecture as a function of model depth. For the regression datasets, all architectures benefit from increasing depth up to a point. For GNN models with more than $6$ and $8$ layers for \esol (left) and \lipo (middle) datasets respectively performance starts decreasing. Similarly for JKNet for models with more than $8$ and $10$ layers for \esol and \lipo respectively. On the other hand, with  the exception of the \enzymes dataset, DSGNN performance continues to improve for up to $16$ layers for both datasets before it flattens out. Our evidence suggests that for graph-level tasks % but perhaps depended on the dataset, 
DSGNNs can exploit larger model depth to achieve improved performance when compared to standard GNNs and JKNets.

\subsubsection{Node Classification}
\label{sec:results_node_classification}
Table~\ref{tab:results_summary_node_datasets} shows that the standard GNN architecture outperformed the others in two of the three node classification datasets, namely \cora and \citeseer. DSGNN demonstrated a small advantage on the larger \pubmed dataset. As previously reported in the literature, shallow architectures perform best on these citation networks. We observe the same since for the smaller \cora and \citeseer all architectures performed best with $2$ to $4$ layers. Only on \pubmed all architectures benefited from increased model depth. We attribute this to the graph's larger size where more graph convolutional layers allow for information from larger neighborhoods to inform the inferred node representations. 

It can be seen in Figure~\ref{fig:deep_gnn_node_performance} that for the smaller \cora and \citeseer, for all models performance degrades as model depth increases. As we noted earlier, this performance degradation has been attributed to the over-smoothing problem in GNNs. In our experiments, DSGNN demonstrated consistently higher resilience to over-smoothing than competing methods. 
% but still failed to outperform shallow models.
\Cref{tab:results_summary_node_datasets_25} in the Appendix shows the performance of all architectures with $25$ layers and clearly indicates that DSGNN outperforms the standard GNN and JKNet for \cora and \pubmed. JKNet is best for \citeseer with DSGNN a close second. As expected DSGNN and JKNet are more resilient to over-smoothing as compared to the standard GNN with more than $12$ layers.  For all datasets and especially \citeseer, performance for the standard GNN degrades substantially as a function of model depth.

Lastly, we note that for all datasets the addition of pair normalization \citep[PairNorm,][]{Zhao2020PairNorm} to the standard GNN hurts performance. This finding is consistent with the results in \citet{Zhao2020PairNorm}. However, as we will see in \cref{sec:missing_features}, PairNorm can be beneficial in the missing feature setting. \cref{tab:results_summary_graph_datasets} shows that the performance of GNN with PN drops by approximately $4.7\%, 3.1\%$ on \cora and \citeseer respectively. DSGNN with PairNorm is the worst performing architecture across all node classification datasets. Consequently, we do not recommend the combination of deep supervision and PairNorm. 

\subsubsection{Node Classification with Missing Features}
\label{sec:missing_features}

\Citet{Zhao2020PairNorm} introduced the missing features setting for the node classification task and demonstrated that GNNs with PairNorm achieve the best results and for deeper models. In the missing features setting, a proportion of nodes in the validation and test sets have their feature vectors zeroed. This setting simulates the missing data scenario common in real-world applications. The missing data proportion can vary from $0\%$ where all nodes have known attributes and $100\%$ where all nodes in the validation and test sets have missing attributes. Here we consider the performance of standard GNN, JKNet, and DSGNN for the latter setting only.

Table~\ref{tab:results_summary_node_datasets_mv} and Figure~\ref{fig:deep_gnn_node_mv_performance} show the performance of the three architectures in the missing features setting. We note that in comparison to the results in Table~\ref{tab:results_summary_node_datasets} and excluding \citeseer, all models achieved their best performance at larger depth. Interestingly and in contrast to \citet{Zhao2020PairNorm}, we found that the standard GNN architecture performed best for the smaller \cora and \citeseer graphs. We attribute the standard GNN's good performance to our use of a model with high capacity ($8$ attention heads and $8$-dimensional embeddings for each head) as well as careful tuning of relevant hyper-parameters. \Citet{Zhao2020PairNorm} use a simpler model, e.g., one attention head, and do not tune important hyper-parameters such as learning rate, dropout and weight decay.

However, on the larger \pubmed dataset, DSGNN with $10$ layers achieves the highest test accuracy. A DSGNN model with $25$ layers as shown in Figure~\ref{fig:deep_gnn_node_mv_performance} and Table~\ref{tab:results_summary_node_datasets_25_mv} in the Appendix achieves the highest test accuracy even when compared to the $10$-layer DSGNN model; the latter was selected for inclusion in Table~\ref{tab:results_summary_node_datasets_mv} because it achieved the highest validation accuracy that we used for model selection across model depth. We provide additional analysis of DSGNN's ability to learn more discriminative node representations and alleviate over-smoothing in the Appendix Section \ref{sec:learned-representations}. We conclude that DSGNN is the more robust architecture to the over-smoothing problem in the missing feature setting and especially for larger graphs.
% We see that DSGNN has a small advantage over the standard GNN and JKNet for $3$ out of $4$ datasets namely the two regression datasets ESOL and Lipophilicity as well as Enzymes. For the Proteins dataset the standard GNN outperforms the other two models with DSGNN a close second. Finally, we note the high variance for all methods and datasets, especially for the ESOL dataset indicating that perhaps there is no significant difference between the three architectures. 
%For DSGNN and both datasets using GAT convolutions was the best performer whereas for GNN on ENZYMES and PROTEINS the best were GAT and GCN respectively. These results provide support that parametric neighbourhood aggregation schemes are more expressive than those with fixed weights. 
%Most importantly, however, we note that the readout functions in all cases have been the non-parametric mean and max. For ENZYMES, mean readout was best for both architectures whereas for PROTEINS it was max. GNNs with these readout functions are faster to train since the total number of network parameters is smaller.

% \subsection{Deep GNNs and Over-smoothing}
% \label{sec:deep_gnns}

% We explore the behavior of the different architectures when training deep GNNs and whether DSGNNs can alleviate the over-smoothing problem. Figure~\ref{fig:deep_gnn_graph_performance} shows test RMSE for the Lipophilicity and ESOL datasets as a function of the number of graph convolutional layers for each of the three architectures. The number of layers ranges from $2$ to $20$ increasing by $2$. For this experiment, we have used $64$-dimensional gated attention for graph pooling. We see that performance for JKNet and DSGNN is maintained as the depth increases implying that both models are resilient to over-smoothing. This is not the case for the standard GNN architecture with performance significantly degrading above $8$ and $12$ layers for Lipophilicity and ESOL datasets respectively. Adding more layers does not improve performance with the lowest RMSE achieved with only $4$ layers for all architectures and the Lipophilicity dataset. For ESOL, there is a small benefit going up to $6$ graph convolutional layers. 

% We conclude that deep supervision and jump connections are equally effective in tackling the over-smoothing problem. Furthermore, for graph classification datasets where each graph is small, adding more graph convolutional layers is of no benefit as compared to shallow GNNs.

% \subsubsection{Sub-networks}
% \label{sec:subnetworks} 

% The DSGNN architecture trains a classifier using as input the learnt representations output by each graph convolutional layer. As mentioned before, this encourages the network to learn discriminative representations across all network layers. This implies that the classifiers trained using input from the first few network layers may provide good enough performance, thus making it possible to use only a sub-network for predicting on test data. Such a sub-network has significantly fewer parameters than the full model, reducing the memory requirements and allowing for faster inference time. The same operation cannot be performed when using jump connections. For JKNet, the input vector to the predictive layer is the sum of the vectors output from the readout layers. Thus, removing some of these, results in an input vector to the predictive layer of incorrect magnitude. 

% Let us consider the $4$-layer DSGNN model trained using the Lipophilicity dataset. We compare the performance of the $2$-layer sub-network consisting of the first $2$ out of $4$ layers against the $2$-layer GNN and JKNet models. We note that, as shown in \cref{fig:deep_gnn_performance}, the $4$-layer DSGNN already outperforms the $4$-layer GNN and JKNet models. We use the notation \textbf{DSGNN\_n\_m} where \textbf{n} denotes the number of graph convolutional layers for the full model and \textbf{m} denotes the number of layers in the sub-network starting from the input layer. For GNN and JKNet models we only specify \textbf{n} since it is not possible to extract sub-networks .

% Figure~\ref{fig:sub_net_performance} shows that the $2$-layer sub-network derived from the $4$-layer DSGNN model denoted by DSGNN\_4\_2 outperforms the corresponding GNN\_2 and JKNet\_2 models that have the same number of parameters. All $2$-layer models consist of $2$ GAT layers with the same number of attention heads. We also note that the DSGNN\_4\_2 model performs competitively when compared to the GNN\_4 and JKNet\_4 models; as shown in Table~\ref{tab:model_trainable_parameters}, the latter two have more than twice as many parameters since each has $4$ GAT layers versus the $2$ GAT layers in DSGNN\_4\_2. This provides evidence that when using deep supervision it is possible to train models that achieve high accuracy yet can be simplified to improve inference speed at test time.
% %\todo[inline]{What is the actual gain in terms of memory and computation time? Can we provide numbers or at least theoretical gains? PE: I added table~\ref{tab:model_trainable_parameters} showing the number of trainable parameters for the relevant models} 
% \begin{figure}[t]
% 	\centering
% 	    \begin{tabular}{c}
%         	\includegraphics[width=11.0cm]{figures/sub_net_performance_lipo.pdf} 
%         \end{tabular}
%         \begin{tabular}{l c}
%             \toprule
%             Model & Test RMSE \\ 
%             \midrule
%             DSGNN\_2*             & 0.70 $\pm$ 0.04 \\
%             DSGNN\_2\_1           & 0.77 $\pm$ 0.03 \\
%             DSGNN\_2\_2*          & 0.69 $\pm$ 0.05 \\
%             \textbf{DSGNN\_4}     & 0.65 $\pm$ 0.05 \\
%             DSGNN\_4\_1           & 0.76 $\pm$ 0.04 \\
%             \underline{DSGNN\_4\_2*} & 0.68 $\pm$ 0.07 \\
%             DSGNN\_4\_3           & 0.66 $\pm$ 0.04 \\
%             \textbf{DSGNN\_4\_4}  & 0.65 $\pm$ 0.04 \\
%             GNN\_2*               & 0.71 $\pm$ 0.08 \\
%             GNN\_4                & 0.68 $\pm$ 0.05 \\
%             JKNet\_2*             & 0.70 $\pm$ 0.05 \\
%             JKNet\_4              & 0.67 $\pm$ 0.05 \\
%             \bottomrule
%         \end{tabular}
%     \caption{Performance comparison of GNN, JKNet, and DSGNN architectures against DSGNN sub-networks on the Lipophilicity dataset. Performance is the RMSE averaged over $10$ runs. We use the notation DSGNN\_n\_m such that n is the number of layers in the full model and m the number of layers in the sub-network starting from the input layer. For GNN and JKNet we only specify n. The actual mean performance and standard deviation for each model is  shown in the table on the right. We use * to denote the $2$-layer models with equal number of parameters. The overall best performing model is shown in bold and the best performing $2$-layer model is underlined.}
% 	\label{fig:sub_net_performance}
% \end{figure}
% \begin{table}
%     \centering
%     \begin{tabular}{l  c  c  c}
%         \toprule
%         Model & Layers  & Layers    & Trainable Parameters \\ 
%               & (All)   & (Sub-net) &  \\ 
%         \midrule
%         $GNN$      &  2  &  - &  1,266,241 \\        
%         $GNN$      &  4  &  - &  3,363,393 \\
%         $JKNet$    &  2  &  - &  1,331,841 \\
%         $JKNet$    &  4  &  - &  3,560,193 \\ 
%         $DSGNN$    &  4  &  - &  3,561,732 \\
%         $DSGNN$    &  4  &  3 &  2,314,817 \\
%         $DSGNN$    &  4  &  2 &  1,266,241 \\         
%         \bottomrule
%     \end{tabular}
%     \caption{Number of trainable parameters for the GNN, JKNet and DSGNN model architectures. For DSGNN, we include the number of parameters for the full $4$-layer model and the $2$ and $3$-layers sub-networks.}
%     \label{tab:model_trainable_parameters}
% \end{table}


==> content/preamble_icml.tex <==
% THINGS INCLUDED IN THE ICML TEMPLATE 

\usepackage[usenames,dvipsnames]{xcolor} % EVB 

\usepackage{icml2022}

% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{booktabs} % for professional tables

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2022} with \usepackage[nohyperref]{icml2022} above.
% \usepackage{hyperref}

\usepackage[colorlinks,linktoc=all]{hyperref} % EVB


% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}

% Use the following line for the initial blind version submitted for review:
\usepackage{icml2022}

% If accepted, instead use the following line for the camera-ready submission:
% \usepackage[accepted]{icml2022}

% For theorems and such
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}

% if you use cleveref..
\usepackage[capitalize,noabbrev]{cleveref}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

% Todonotes is useful during development; simply uncomment the next line
%    and comment out the line below the next line to turn off comments
%\usepackage[disable,textsize=tiny]{todonotes}
\usepackage[textsize=tiny]{todonotes}

\icmltitlerunning{Deeply-Supervised GNNs}

==> content/title.tex <==
\twocolumn[
%\icmltitle{Deeply-Supervised Graph Neural Networks}
% \icmltitle{Deeply-Supervised Graph Neural Networks: Tackling the over-smoothing problem for graph and node property prediction tasks}
%\icmltitle{Deeply-Supervised Graph Neural Networks}
\icmltitle{Addressing Over-Smoothing in Graph Neural Networks via Deep Supervision}

% It is OKAY to include author information, even for blind
% submissions: the style file will automatically remove it for you
% unless you've provided the [accepted] option to the icml2022
% package.

% List of affiliations: The first argument should be a (short)
% identifier you will use later to specify author affiliations
% Academic affiliations should list Department, University, City, Region, Country
% Industry affiliations should list Company, City, Region, Country

% You can specify symbols, otherwise they are numbered in order.
% Ideally, you should not use this facility. Affiliations will be numbered
% in order of appearance and this is the preferred way.
\icmlsetsymbol{equal}{*}

\begin{icmlauthorlist}
\icmlauthor{Pantelis Elinas}{equal,comp}
\icmlauthor{Edwin V. Bonilla}{equal,comp}
\end{icmlauthorlist}

\icmlaffiliation{comp}{CSIRO's DATA61, Sydney, AU}

\icmlcorrespondingauthor{Pantelis Elinas}{pantelis.elinas@data61.csiro.au}
%\icmlcorrespondingauthor{Firstname2 Lastname2}{first2.last2@www.uk}

% You may provide any keywords that you
% find helpful for describing your paper; these are used to populate
% the "keywords" metadata in the PDF but will not be shown in the document
\icmlkeywords{Graph Neural Networks, deep supervision, representation learning}

\vskip 0.3in
]

% this must go after the closing bracket ] following \twocolumn[ ...

% This command actually creates the footnote in the first column
% listing the affiliations and the copyright notice.
% The command takes one argument, which is text to display at the start of the footnote.
% The \icmlEqualContribution command is standard text for equal contribution.
% Remove it (just {}) if you do not need this facility.

%\printAffiliationsAndNotice{}  % leave blank if no need to mention equal contribution
\printAffiliationsAndNotice{\icmlEqualContribution} % otherwise use the standard text.

